Image Retrieval from Contextual Descriptions

The ability to integrate context, including perceptual and temporal cues, plays a pivotal role in grounding the meaning of a linguistic utterance. In order to measure to what extent current vision-and-language models master this ability, we devise a new multimodal challenge, Image Retrieval from Contextual Descriptions (ImageCoDe). In particular, models are tasked with retrieving the correct image from a set of 10 minimally contrastive candidates based on a contextual description. As such, each description contains only the details that help distinguish between images. Because of this, descriptions tend to be complex in terms of syntax and discourse and require drawing pragmatic inferences. Images are sourced from both static pictures and video frames. We benchmark several state-of-the-art models, including both cross-encoders such as ViLBERT and bi-encoders such as CLIP, on ImageCoDe. Our results reveal that these models dramatically lag behind human performance: the best variant achieves an accuracy of 20.9 on video frames and 59.4 on static pictures, compared with 90.8 in humans. Furthermore, we experiment with new model variants that are better equipped to incorporate visual and temporal context into their representations, which achieve modest gains. Our hope is that ImageCoDE will foster progress in grounded language understanding by encouraging models to focus on fine-grained visual differences.

==> todos.tex <==
Reviews: https://openreview.net/forum?id=ObaBB7DvM4

MAR 25:
Agenda for Siva:
1. short-term timeline: Monday Samsung dry run (3 days), be Arxiv ready by end of next week (~7 days), 5th April (11 days), 12th April NLP group talk (18 days), prepare ACL talk, finishing course work around end of April
2. content of talk (look at old slides)
    - what is the main idea/motivation? what should be mentioned in a 2 minute elevator talk?
    - is NLP group talk 30 min or 60 min?
3. Get to Arxiv ready state
    - should i put on arxiv when everything is perfect aka "tweetable" or should i put it there now, then work on more stuff and then tweet about it in a week?
    - website/repo: explain data format on README better, display leader board and examples
    - leaderboard: eval.ai or competitions.codalab.org/competitions/ or without any?
    - tweet

MAR 13:
A1. Did you describe the limitations of your work?
 - while we claim pragmatic model would help/make sense, we do not show that by modeling pragmatics we get better results
 - single run per hyperparameter setting due to trying many different variants, run times and focus on resource paper and analysis

Data collection:
 - we adopt license of underlying data and MIT license for our own collected descriptions.
 - worker pay see Appendix


MAR 12:
Licensing:
-------
open-images:
Apache License 2.0
Permissions
 Commercial use
 Modification
 Distribution
 Patent use
 Private use
Limitations
 Trademark use
 Liability
 Warranty
--------
volta:
This work is licensed under the MIT license. See LICENSE for details. Third-party software and data sets are subject to their respective licenses.
--------
NLVR2:
We have licensed the annotations of the NLVR2 images (sentences and binary labels) under CC-BY-4.0 (https://creativecommons.org/licenses/by/4.0/). We do not license the NLVR2 images as we do not hold the copyright to them.
-------
YouCook: MIT License? YouCook2 is MIT license so YouCook prob as well
------
msr-vtt:
no license mentioned?
-----
video-storytelling:
 Creative Commons Attribution 4.0 International



MAR 11:
left todos:
licensing on github (look for 4 image/vid sources, volta license)
ethics section
acknowledgements

stuff that siva said



explain data format on README better

potentially switch to Zonodo

MAR 9:

Siva says:

use this for leaderboard:
https://eval.ai/
or: https://competitions.codalab.org/competitions/

static examples on website is fine!
integrate leaderboard from eval.ai into website, i.e. by fetching json/csv from it
for leaderboard give people test set without answers

arxiv in 2-3 weeks with leaderboard
tweet

------

Yay! I accomplished most things for today and for the rest it is only repo and website!

8 MAR: 
What is still left to do? 

show red parts to Siva
http://langcog.stanford.edu/papers_new/goodman-2016-tics.pdf

explain UNITER (1-4h)
    lookup wandb -> params note them down on paper
    writeup

repo and website

prep tweet?

FEB 28:
------------------------------------------------------------------------------------------
general priorities/chronological task order:
- UNITER/ViLBERT scores

- refExpr in related work: "the type of reasoning and skills involve resemble the well-established task of RefExpr where the reasoning happens in a single image etc."

- in intro: "when we say context we mean that by examining our examples we see they often require drawing cues and connecting several images in complex ways, more so than many other established datasets"

- in rel work re pragmatics: "while we do not model pragmatics explicitly many of our examples are easier to solve if a model considers the speakers intention of selecting exactly 1 image and not several, such as fig X (no bridesmaid at all) -> semantically perhaps correct for 2-3 images but since we know speaker only tries to narrow it down to 1, it has to be this one. We saw many such examples, often related to adjectives along a scale (gradable?), i.e. "the man is looking down" -> is looking down in 2 images but in one he is looking down "more".

- fix kappa agreement

- look into LXMBERT comment:

- add github/website link to introduction

- Acknowledgements!
-----------------------------------------------------------------------------------------

Full notes:
- Ref expressions
    "mention the connection to referring expressions somewhere in the paper"
    Yu, Licheng, et al. "Modeling context in referring expressions." European Conference on Computer Vision. Springer, Cham, 2016. Mao, Junhua, et al. "Generation and comprehension of unambiguous object descriptions." Proceedings of the IEEE conference on computer vision and pattern recognition. 2016.
    https://arxiv.org/abs/1511.02283 April 2016
    
    I believe the presentation of the dataset would benefit from a comparison to the approach used by Kazemzadeh et al (EMNLP; 2014) for ReferIt Game (the precursor to Ref-COCO etc), where a similar describe-and-identify paradigm was used, albeit in a more gamified setting and with the goal of identifying objects/regions within images, rather than images from a set. This is a widely-used dataset in the community, and attention should be drawn to the similarities and differences. More generally, the task described here shares a number of characteristics with the task of referring expression generation, where identification-in-context is the key goal. This literature should be discussed.
    https://aclanthology.org/D14-1086/ Kazemzadeh et al (EMNLP; 2014)
    Aug 2016 follow-up: https://arxiv.org/pdf/1608.00272v3.pdf


    
- refining the intro/notion of context a bit
The only thing I can complain about is the rather general framing of the dataset in the introduction. To me, it seems that "contextual descriptions" is a bit too vague and generic as a term for describing the contribution. The contexts explored in this work are very specific distractor-like types of contexts where an image appears in combination with extremely similar images. This is close to the classical referring expression setting that investigates descriptions of objects in the context of similar distractor objects. The resulting expressions may be called discriminative descriptions/unambiguous references or something along these lines.

- in table 5 could present the human results directly, instead of having the reader need to flip back to compare
- figure 4 could include human accuracy on these subsets

- CLIP is said to outperform ViLBERT due to more parameters and more training data. While the training data aspect is almost certainly a factor, on some tasks, CLIP has been found to outperform models couched in the more familiar dual-stream architecture (such as LXMERT) despite the fact that these are larger in terms of paramterisation (see, as an example of such results, the comparison of CLIP against 2 other models here: https://arxiv.org/abs/2109.07301). What might also contribute to cLIP's performance is its contrastive learning objective (https://arxiv.org/pdf/2103.00020.pdf)

- The observation that more improvement is seen on video compared to static images after the inclusion of context modules is well--taken. This, however, seems to arise from an artefact of the dataset itself: static images are unrelated, but similar; video frames are related insofar as they are sampled from the same stream. In short, one wonders if the notion of "context" for static images is somewhat weaker. Some discussion of this would be useful.

- The dataset and task are motivated on pragmatic grounds, but the justification for this is somewhat thin. Of course, context is key to resolving the retrieval task presented, but Section 1 also makes reference to "speaker intention" which, as far as this reviewer can see, is nowhere really considered (the experimental setup only focuses on the use of context, not speaker intention, which is merely implicit). My point here is that the grounds for such claims need to be made clearer, otherwise they appear somewhat spurious.

- On p. 8, "Error analysis" you say you used Pearson's correlation, but the notation suggests Spearman's rho (Pearson's is usually denoted r). Please check.



JAN 31:
First todo: add referring expressions into related work
Second todo: explain why it is pragmatic a bit more (reference to gricean maxims eg)



1. distribute data
    - github repo
        - fix experiment code
    - huggingface datasets
    - website for dataset
    - datasheet
    - paperswithcode
    - create leaderboard?
    
2. come up with new name?
nope not gonna happen lol

3. put validation results in appendix

4. run UNITER


We thank all our reviewers for their positive and detailed reviews!
 
 We took several valuable suggestions and comments away from the reviews that we would like to briefly address here:
 
 R2 is correct that ImageCoDe has parallels with NLVR2. But while another task may also involve several images (which many other datasets i.e. in pragmatic captioning also do), a new task can still differ in many other aspects. As vision-and-language is becoming a larger and larger field, it is reasonable to adopt more fine-grained distinctions between tasks and capabilities, just like in NLP where QA might have been a specific task by itself and now has many different variants and subtasks that test different capabilities or phenomena.
 We differ from NLVR2 in several ways:
An NLVR2 description indicates whether the description is true for a pair of images or not, a binary classification task. Our task is a retrieval task. We have to retrieve the right image from a set of 10 images.
Our descriptions in most cases can also work as stand-alone captions, whereas this does not hold in NLVR2. 3. The majority of our images come from videos, whereas NLVR2 has only static images.
 
 In the final paper we will make a more explicit comparison to the analogous research on referring expressions (R1,R3).
 
We also agree that the language in ImageCoDe would not exactly be seen in real tasks (just like the NLVR2 task is quite constructed in some sense). However we do believe interesting broader skills are tested with the used language that will be needed for "real tasks", albeit in slightly different linguistic form.

 Finally, we are thankful to R3 for pointing out that single-stream models are a third distinct family of models whose processing of two modalities could be qualitatively different and perhaps even more contextual. We will therefore additionally evaluate a model like UNITER.

Also, Benderrule?
